Quotable Signatures for Authenticating Shared Quotes

Quotable signature schemes are digital signature schemes with the additional property that from the signature for a message, any party can extract signatures for (allowable) quotes from the message, without knowing the secret key or interacting with the signer of the original message. Crucially, the extracted signatures are still signed with the original secret key. We define a notion of security for quotable signature schemes and construct a concrete example of a quotable signature scheme, using Merkle trees and classical digital signature schemes. The scheme is shown to be secure, with respect to the aforementioned notion of security. Additionally, we prove bounds on the complexity of the constructed scheme and provide algorithms for signing, quoting, and verifying. Finally, concrete use cases of quotable signatures are considered, using them to combat misinformation by bolstering authentic content on social media. We consider both how quotable signatures can be used, and why using them could help mitigate the effects of fake news.

==> tex/instantiation.tex <==
\section{Quotable Signatures for Text Based Media}\label{sec:qsfortex}

% This is our concrete use case where we apply quotable signatures to sharing
% quotes from news medias to social medias.
In the previous section, we defined quotable signatures and realised them
using Merkle trees. In this section, we will turn our attention to a concrete
example of where quotable signatures can be useful, namely using an
instantiation of quotable signatures for text, as part of a scheme for
verifying the authenticity of quotes from text based news media. We
introduce this instantiation in \cref{ssec:fight-fn} and consider how
it could fit into the existing infrastructure and current workflow for
journalists in \cref{ssec:in-current-world}.

% Text, multiple examples and this as a specific example. Refer to 'from our
% talks with Danish media compnaies' would fit so and so. Say how it is not
% only way to use it, name other uses.

\subsection{Promoting Authentic Content}\label{ssec:fight-fn}
% The idea more concretely, with explanation of how it fits in. If we go for
% DDC-ish venue, we will probably want to call this something else.
As we discussed in the introduction, disinformation (\textquote{fake news}) is
a major challenge that our society faces, which cannot be solved by just (manually
or automatically) flagging (potential)
disinformation~\cite{2020ERCom...2h1003D,doi:10.1177/1529100612451018,10.1007/978-3-030-61841-4_16}.
Our proposal is to use quotable signatures for text, supplementing the flagging of
problematic content,  authenticating the source of quotes from
news articles, and potentially other sources. Using quotable signatures allows users
that share quotes from sources supporting quotable signatures to include
signatures for their quotes, which in turn enables those who read the quotes to
verify the source and authenticity of the quoted text. In the case where the source is
a news article, the terms from \cref{ssec:q-s-setting} would correspond
to the news provider being the Signer, the one making the quote being the
Quoter, and the reader of the quote being the Verifier.

Since applications of quotable signatures are in no way limited to news media,
we will
continue to use the generic terms for the parties. However, we note that using
quotable signatures to verify the authenticity of the source of a quote from a
news article is an application that has the potential to be effective in
combating disinformation. To quote Urban and
Schweiger~\cite{doi:10.1080/1461670X.2013.856670}: \enquote{Furthermore, media
  brand images proved to be an important heuristic when recipients have to
  evaluate news quality.} Hence, providing a guarantee about what news media
the source originates from could help the reader/Verifier to decide whether or not to trust
the quote.

\subsection{Quotable signatures in the current
  infrastructure}\label{ssec:in-current-world}
In this section we consider how challenging it is to implement quotable
signatures into the existing workflow and infrastructure used by news media
companies. %In addition to the cited literature,
These considerations are informed by talks with a %Danish
news media
company. Specifically, we talked with the editor in charge of the platforms and
the editor in charge of the digital editorial office at
% one of the largest Danish
a large media company that is producing multiple newspapers for different
regional areas, in both paper and digital versions. While technically a
commercial meida company, this company has a publicist approach to news making
and a history of engaging with communities to support the public democratic
debate.
%We emphasize that despite
%their size, and the number of different newspapers they operate, this is only
%one company, and is therefore not representative, but serve only to show that it
%is not an infeasible task to integrate quotable signatures with current systems
%used by news media companies.
%Therefore, it makes sense to implement a
%real-world prototype, for further testing.

From our discussions, it is clear that the current workflow employed by modern
media companies is already highly automated and it appears that it should be
quite simple to integrate a process by which, when an article is published (or
updated), it is automatically signed with the media company's public key. In
general, it should be conceptually simple to implement a system to automatically
take on the role of a Signer for parties that host their own content. For
parties that have their content hosted by a third party, more sophisticated
solutions might be needed.

With regards to the infrastructure needed to use quotable signatures, we
observe that there are two main challenges with using quotable signatures:
distributing signatures and distributing (and authenticating) public keys. The
latter challenge can be solved by either implementing a public key
infrastructure (PKI) specifically for an application of quotable signatures,
or by tapping into one of the existing PKIs that are
e.g., integrated into operating systems and web browsers.
%, such as the Transport Layer Security (TLS)
%protocol, that already exists to provide authenticity (amongst other
%guarantees) for communications over computer networks.
%% RN: TLS is not a PKI.
The advantage of the
second approach is that the infrastructure already exists and is widely
adopted, with (almost) every organization with their own website already
having a private key.
% The disadvantage is that many organizations that do not
% host their own website might not be in possession of their private key and that
% obtaining a private key for this PKI requires having a website.
%% RN: I am not sure if these statements on disadvantages are true.
% For the
% challenge of distributing (and storing) signatures for quotes, we note that we
% are not aware of any preexisting infrastructure that can be directly adopted.
%% RN: The world wide web should do.
For the first challenge, we note that the ideal solution would be for the party
hosting the quote to also provide support for including a location for
signature, but, as we will argue in \cref{sssec:platform-independence}, an
approach not requiring their support is also possible.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

